Self-supervised Depth Denoising Using Lower- and Higher-quality RGB-D sensors

Consumer-level depth cameras and depth sensors embedded in mobile devices enable numerous applications, such as AR games and face identification. However, the quality of the captured depth is sometimes insufficient for 3D reconstruction, tracking and other computer vision tasks. In this paper, we propose a self-supervised depth denoising approach to denoise and refine depth coming from a low quality sensor. We record simultaneous RGB-D sequences with unzynchronized lower- and higher-quality cameras and solve a challenging problem of aligning sequences both temporally and spatially. We then learn a deep neural network to denoise the lower-quality depth using the matched higher-quality data as a source of supervision signal. We experimentally validate our method against state-of-the-art filtering-based and deep denoising techniques and show its application for 3D object reconstruction tasks where our approach leads to more detailed fused surfaces and better tracking.

==> figs/some_examples.tex <==
\begin{figure*}
    \centering
    \newlength{\mdda}
    \setlength{\mdda}{2.1cm}
    \centering\resizebox{0.95\linewidth}{!}{
    \begin{tabular}{@{}ccccccc@{}}
    
    
    \includegraphics[width=\mdda]{figs/images/for_some_examples/pic1/c.png} &
    \includegraphics[width=\mdda]{figs/images/for_some_examples/pic1/d.png} & 
    \includegraphics[width=\mdda]{figs/images/for_some_examples/pic1/dr.png} &
    
    \includegraphics[width=\mdda]{figs/images/for_some_examples/pic1/c2.png} &
    \includegraphics[width=\mdda]{figs/images/for_some_examples/pic1/d2.png} & 
    \includegraphics[width=\mdda]{figs/images/for_some_examples/pic1/dr2.png} &
    \\ 
    
    \includegraphics[width=\mdda]{figs/images/for_some_examples/pic2/c.png} &
    \includegraphics[width=1.2cm]{figs/images/for_some_examples/pic2/d.png} & 
    \includegraphics[width=1.2cm]{figs/images/for_some_examples/pic2/dr.png} &
    
    \includegraphics[width=\mdda]{figs/images/for_some_examples/pic2/c2.png} &
    \includegraphics[width=1.3cm]{figs/images/for_some_examples/pic2/d2.png} & 
    \includegraphics[width=1.3cm]{figs/images/for_some_examples/pic2/dr2.png} &
    \\ 
    
    \includegraphics[width=\mdda]{figs/images/for_some_examples/pic3/c.png} &
    \includegraphics[width=1.5cm]{figs/images/for_some_examples/pic3/d.png} & 
    \includegraphics[width=1.5cm]{figs/images/for_some_examples/pic3/dr.png} &
    
    \includegraphics[width=\mdda]{figs/images/for_some_examples/pic3/c2.png} &
    \includegraphics[width=1.6cm]{figs/images/for_some_examples/pic3/d2.png} & 
    \includegraphics[width=1.6cm]{figs/images/for_some_examples/pic3/dr2.png} &
    \\ 
    
    \includegraphics[width=\mdda]{figs/images/for_some_examples/pic5/c.png} &
    \includegraphics[width=1.1cm]{figs/images/for_some_examples/pic5/d.png} & 
    \includegraphics[width=1.1cm]{figs/images/for_some_examples/pic5/dr.png} &
    
    \includegraphics[width=\mdda]{figs/images/for_some_examples/pic5/c2.png} &
    \includegraphics[width=1.8cm]{figs/images/for_some_examples/pic5/d2.png} & 
    \includegraphics[width=1.8cm]{figs/images/for_some_examples/pic5/dr2.png} &
    \\
    
    \includegraphics[width=\mdda]{figs/images/for_some_examples/pic4/c.png} &
    \includegraphics[width=1.6cm]{figs/images/for_some_examples/pic4/d.png} & 
    \includegraphics[width=1.6cm]{figs/images/for_some_examples/pic4/dr.png} &
    
    \includegraphics[width=\mdda]{figs/images/for_some_examples/pic4/c2.png} &
    \includegraphics[width=1.1cm]{figs/images/for_some_examples/pic4/d2.png} & 
    \includegraphics[width=1.1cm]{figs/images/for_some_examples/pic4/dr2.png} &
    \\
    
    \includegraphics[width=\mdda]{figs/images/for_some_examples/pic6/c.png} &
    \includegraphics[width=1.8cm]{figs/images/for_some_examples/pic6/d.png} & 
    \includegraphics[width=1.8cm]{figs/images/for_some_examples/pic6/dr.png} &
    
    \includegraphics[width=\mdda]{figs/images/for_some_examples/pic6/c2.png} &
    \includegraphics[width=1.6cm]{figs/images/for_some_examples/pic6/d2.png} & 
    \includegraphics[width=1.6cm]{figs/images/for_some_examples/pic6/dr2.png} &
    \\ %\vspace*{-4mm}
    
    
    
    \small{(a) Color} & \small{(b) TD} & \small{(c) Ours (basic)} & \small{(d) Color} & \small{(e) TD} & \small{(f) Ours (basic)}
    \end{tabular}}
    \vspace*{3mm}\caption{More examples produced by our model for various people and environments. Here we use the basic model $\U$ model as no sequential data is available.}\label{fig:comparison_reb}
\end{figure*}

==> figs/teaser_old.tex <==
\begin{figure}
\centering
\begin{tabular}{ cccccc}%m{4cm}  m{2.7cm} m{2.7cm}   m{2.7cm}  }
    \newlength{\mddc}
    \setlength{\mddc}{1cm}
    \centering
    % \includegraphics[width=.30\textwidth]{figs/setup.jpg} &
    % \includegraphics[width=.15\textwidth]{figs/depth_denoising/seq1/iphonearchive1555929526.05.zip_00574.png} &
    % \includegraphics[width=.15\textwidth]{figs/depth_denoising/seq1/lstmarchive1555929526.05.zip_00574.png} &
    % \includegraphics[width=.15\textwidth]{figs/depth_denoising/seq1/kinect_depth00574.png} &
    % \includegraphics[width=.15\textwidth]{figs/depth_denoising/seq1/kin_enharchive1555929526.05.zip_00574.png} \\
    % (a) & (b) LQ depth & (c) Ours & (d) HQ depth & (e) Ours
    
    % \includegraphics[width=.30\textwidth]{figs/setup.jpg} 
    % (a)  &
    
    
    % \includegraphics[width=.21\textwidth]{figs/images/for_teaser/pic2/00061-1562083973.6927621.jpg}
    \includegraphics[width=.20\textwidth]{figs/images/for_teaser/pic4/00067-1561745076.333075.jpg} &
    
    % \includegraphics[width=.19\textwidth]{figs/images/for_teaser/pic2/original_iphone_oldseq6_00061-1562083973.png} 
    \includegraphics[width=.16\textwidth]{figs/images/for_teaser/pic4/original_iphone_oldseq7_00067-1561745076.png} &
    
    % \includegraphics[width=.19\textwidth]{figs/images/for_teaser/pic2/unet_new_valseq6_00061-1562083973.png} 
     
    
    \includegraphics[width=.16\textwidth]{figs/images/for_teaser/pic4/rgfseq7_00067-1561745076.png} &
    
    \includegraphics[width=.16\textwidth]{figs/images/for_teaser/pic4/drr_iphoneseq7_00067-1561745076.png} &
    
    \includegraphics[width=.16\textwidth]{figs/images/for_teaser/pic4/unet_new_valseq7_00067-1561745076.png}
    
    \\
    \includegraphics[width=.21\textwidth]{figs/images/for_teaser/pic2/00061-1562083973.6927621.jpg}&
    
    \includegraphics[width=.19\textwidth]{figs/images/for_teaser/pic2/original_iphone_oldseq6_00061-1562083973.png} &
    
    \includegraphics[width=.19\textwidth]{figs/images/for_teaser/pic2/rgfseq6_00061-1562083973.png} &
    
    \includegraphics[width=.19\textwidth]{figs/images/for_teaser/pic2/drr_iphoneseq6_00061-1562083973.png} &
    
    \includegraphics[width=.19\textwidth]{figs/images/for_teaser/pic2/unet_new_valseq6_00061-1562083973.png} &
    
    \\
    %  \vspace*{-4mm}
    \small{(a) Color} & \small{(b) TrueDepth (TD)} &  \small{(c) RGF}  & \small{(d) DRR} & \small{ (e) Ours(basic)}
    \\
    
\end{tabular}
    \caption{Our model learned in a self-supervised way   takes color and depth data coming from the sensor of an iPhone X as input (a, b) and produces a denoised and refined depth (e). Our method works significantly better than filtering-based (c) and other data-driven approaches (d). We intentionally visualize depth slightly rotated in 3D to highlight the differences between the methods.}\label{fig:teaser}
\end{figure}

% Our method performs denoising and refinement of noisy data coming from TrueDepth sensor of an Iphone X.

